$HS^2$: Active Learning over Hypergraphs

We propose a hypergraph-based active learning scheme which we term $HS^2$, $HS^2$ generalizes the previously reported algorithm $S^2$ originally proposed for graph-based active learning with pointwise queries [Dasarathy et al., COLT 2015]. Our $HS^2$ method can accommodate hypergraph structures and allows one to ask both pointwise queries and pairwise queries. Based on a novel parametric system particularly designed for hypergraphs, we derive theoretical results on the query complexity of $HS^2$ for the above described generalized settings. Both the theoretical and empirical results show that $HS^2$ requires a significantly fewer number of queries than $S^2$ when one uses $S^2$ over a graph obtained from the corresponding hypergraph via clique expansion.

==> lemmascq1.tex <==
\begin{proof}
The following proof is identical to the proof of lemma 1 in \cite{dasarathy2015s2}, we include it here for completeness.\\
Let $\mathcal{E}$ denote that the event that there exists a component $V_i$ such that $V_i\cap L=\emptyset$.. Then by union bound we have 
\begin{align*}
\mathbb{P}[\mathcal{E}]&\leq \sum_{i=1}^{T}\mathbb{P}[V_i\cap L=\emptyset]\\
&\leq \sum_{i=1}^{T}\frac{\binom{n-|V_i|}{|L|}}{\binom{n}{|L|}}\\
&\leq T\frac{\binom{(1-\beta)n}{|L|}}{\binom{n}{|L|}}\\
&\leq T(1-\beta)^{|L|}\\
&\leq \frac{1}{\beta}(1-\beta)^{|L|}
\end{align*}
Note that $T\leq \frac{1}{\beta}$ which can be easily shown from the definition. To conclude, we observe that if we pick $|L|$ as stated in the lemma, then the RHS of the above equation drop below $\alpha$. Hence we complete the proof.
\end{proof}

==> lmaKLbound.tex <==
\begin{proof}
    By definition we have $D(x||y) = x\log \frac{x}{y} + (1-x)\log \frac{1-x}{1-y}$. Then note that we have the following to lower bound for log
    \begin{equation*}
       \begin{split}
            & \log(1+z) \geq z-\frac{z^2}{2} \;\forall |z|<1 \\
            & \log(z) \geq 1-\frac{1}{z}\;\forall z>0
       \end{split}
    \end{equation*}
    We can see them directly by Taylor expansion. Hence applying the first inequality to $\log(\frac{x}{y})$ and the second to $\log\frac{1-x}{1-y}$ we have
    \begin{equation*}
      \begin{split}
           & D(x||y) \geq x(\frac{x-y}{y}-\frac{(x-y)^2}{2y^2}) + (1-x)(1-\frac{1-y}{1-x}) \\
           & = -\frac{x}{2}\frac{(y-x)^2}{y^2}+(y-x)(1-\frac{x}{y}) \\
           & = \frac{(y-x)^2}{y}(1-\frac{x}{2y}) \\
           & \geq \frac{(y-x)^2}{y}(1-\frac{1}{2})\;\text{Since }x\leq y\in[0,1] \\
           & = \frac{(y-x)^2}{2y}
      \end{split}
    \end{equation*}
\end{proof}

==> sec_algoandtheo.tex <==
In this section, we first state the original result for $S^2$ algorithm (\cite{dasarathy2015s2}) on the problem of binary classification. They work with the oracle that can directly return the label for any queried node. Also, they work with the standard graph undirected graph only. Since in their noisy setting, they assume that they could get an i.i.d. answers for the same queried node and using naive majority voting to lower the error probability, we will only present thier noiseless result here.\\
\begin{algorithm2e}
\caption{$S^2$ the noiseless case}\label{alg:S2}
\SetAlgoLined
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwRepeat{Do}{do}{while}
\SetKwInOut{Output}{Output}
\SetKwInput{Mainalgo}{Main Algorithm}
%\SetKwInput{Phaseone}{Phase 1}
%\SetKwInput{Phasetwo}{Phase 2}
  \Input{The graph $G$, query complexity budget $Q(\delta)$
  }
  \Output{The label function $\widehat{f}$
  }
    \Mainalgo{
    $L\leftarrow\phi$\;
    \While{1}{
    $x\leftarrow $ Uniformly at random pick an unlabeled node.\;
    \Do{$x\leftarrow MSSP(G,L)$ exist}{
        Add $(x,f(x))$ to $L$\;
        Remove from $G$ all edges whose two ends have different label.\;
        \If{$|L|= Q(\delta)$}{
            Return \emph{LabelCompletion}$(G,L)$
        }
    }
    }
  }
\end{algorithm2e}
Note that the subroutine \emph{LabelCompletion}$(G,L)$ is the simple label assignment based on $(G,L)$. If we indeed learn the cut set $C$, then $G$ will be the graph such that removing all edges in $C$ and hence we could easily assign labels for the rest nodes according to $(G,L)$. Now we introduce the other key subroutine $MSSP(G,L)$.
\begin{algorithm2e}
\caption{MMSP}\label{alg:MMSP}
\SetAlgoLined
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwRepeat{Do}{do}{while}
\SetKwInOut{Output}{Output}
\SetKwInput{Mainalgo}{Main Algorithm}
%\SetKwInput{Phaseone}{Phase 1}
%\SetKwInput{Phasetwo}{Phase 2}
  \Input{The graph $G$, Label list $L$
  }
  \Output{The midpoint of shortest-shortest path $x$.
  }
    \Mainalgo{\;
        \For{each $v_i,v_j\in L$ such that $f(v_i)\neq f(v_j)$}{
        $P_{i,j}\leftarrow $ shortest path between $v_i,v_j$ in $G$.\;
        $l_{i,j}\leftarrow $ length of $P_{i,j}$.($=\infty$ if doesn't exist)\;
        }
        $(i^*,j^*) = \arg\min l_{i,j}$\;
        \uIf{$(i^*,j^*)$ exists }{
            Return midpoint of $P_{i^*,j^*}$.(Break tie arbitrarily)\;
        }
        \Else{
            Return $\phi$\;
        }
    }

\end{algorithm2e}
To introduce the theoretical guarantee of this algorithm, we will need to introduce some definitions which can characterize the hardness of this task. Assume that the label function $f$ partition $V$ into $T$ connected components $V_1,...,V_T$. This will naturally induce a partition of the cut set $C=\bigcup_{1\leq r<s\leq T}C_{rs}$ where $C_{rs} = \{(x,y)\in C:x\in V_r,y\in V_s\}$. In \cite{dasarathy2015s2} they denote the number of non-empty subsets $C_{rs}$ by $m$ and they call $C_{rs}$ as a cut component. Moreover, we will need the following definitions
\begin{definition}[Balancedness]
    We will assume that the graph $G$ satisfy the following $\beta = \min_{i\in[k]}\frac{|V_i|}{n}$.
\end{definition}
\begin{definition}[Distance between cut edges]\label{def:clusteringofCC}
    Let $d_{sp}^{G}(x,y)$ denote the shortest path between $x,y$ with respect to graph $G$. Let $\Delta:C\times C\rightarrow\mathbb{N}\cup\{0,\infty\}$. Let $e_1 = (x_1,y_1), e_2 = (x_2,y_2)\in C$ such that $f(x_1) = f(x_2)$, $f(y_1) = f(y_2)$ and $f(x_1) \neq f(y_1)$. Then we have
    \begin{equation*}
      \Delta(e_1,e_2) = d_{sp}^{G-C}(x_1,x_2) + d_{sp}^{G-C}(y_1,y_2) + 1
    \end{equation*}
    where $G-C$ denotes the graph $G$ with edges in $C$ are removed. Clearly $\Delta(e_1,e_2) < \infty$ if and only if $e_1,e_2$ lies in the same cut component.
\end{definition}
Let $H_r = (C,\mathcal{E})$ be the "meta-graph" whose vertices are the cut-edge of $G$ and $(e,e')\in\mathcal{E}$ if and only if $\Delta(e,e')\leq r$. Clearly for any $r$, $H_r$ will have at least $m$ connected components.
\begin{definition}\label{def:kappaclustered}
    A cut-set $C$ is said to be $\kappa$-clustered if $H_{\kappa}$ has exactly $m$ connected component. Note that these connected component correspond to the cut components.
\end{definition}
Now we're ready to state the theoretical guarantee of the algorithm~\ref{alg:S2}.
\begin{theorem}[Main theorem in \cite{dasarathy2015s2}]\label{thm:1}
  Suppose $G=(V,E)$ and $f$ are such that the induced cut set $C$ has $m$ cut components that are $\kappa$-clustered. Then for any $\delta>0$, the algorithm~\ref{alg:S2} will recover $C$ with probability at least $1-\delta$ if
  \begin{align*}
  	& Q(\delta) \geq \frac{\log(1/(\beta\delta))}{\log(1/(1-\beta))}\\
    & +m(\lceil\log_2(n)-\log_2(\kappa)\rceil) + |\partial C| (\lceil\log_2(\kappa)\rceil+1)
  \end{align*}

\end{theorem}
\begin{remark}
    Note that in the paper \cite{dasarathy2015s2}, they consider only the binary classification problem but they allow to have $T$ underlying connected components where $T\leq \lfloor\frac{1}{\beta}\rfloor$. We can show that for the $k$-way classification problem the query complexity will be exactly the same if $k\leq T$. Note that it's impossible to have a case $T<k$ by definition.
    Hence the intrinsic hardness will not depends on $k$ once we fix $T$ (or using its upper bound $\frac{1}{\beta}$).
\end{remark}
%\begin{remark}
%    Note that the first term $\frac{\log(1/(\beta\delta))}{\log(1/(1-\beta))}$ can be improved to be %$\frac{\log(m/\delta)}{\log(1/(1-\beta))}$. This is because they use $1/\beta$ as the number of bad events for the union bound, which in %fact can be $m$. One can easily find that $1/\beta \geq m$ and the equality hold only if $G$ is perfectly balanced.
%\end{remark}
\begin{remark}
	If one check the proof in \cite{dasarathy2015s2} carefully, they upper bound the total number of "runs" $R$ by $|\partial C|$, which can in fact bounded by $\min(|C|,|\partial C|)$ which is slightly smaller. This will be proved in the proof of theorem \ref{thm:pairwise}. The main intuition is the upper bound of the number of "runs" $R$ can be either $|C|$ or $|\partial C|$. In the original $S^2$ paper \cite{dasarathy2015s2} they argue that the each "run" will end when a new boundary vertex is found hence $R\leq|\partial C|$. However we observe that a new boundary vertex is found if and only if to (at least) a new cut edge is found. Hence we also have $R\leq |C|$. Hence we have $R\leq \min(|C|,|\partial C|)$. See more details in the proof of theorem \ref{thm:pairwise} and the proof in \cite{dasarathy2015s2}.
\end{remark}

==> sec_conclusion.tex <==
In this final project, we investigate the problem of label prediction on a graph. To be more specific, we design some new algorithms to the settings of same-cluster query, noisy oracle and hypergraph, which are all adapted from the original $S^2$ algorithm. Query complexity of these three settings are derived  and the simulation shows that the gap between the empirical query complexity and theoretical query complexity is reasonable. One interesting direction for the future work is to connect our extensions to the nonparametric active learning i.e. show that our theoretical query complexity is tight for some classes of graph. In addition, more simulations are required to verify our theorems. 

==> sec_noisy.tex <==
In this section, we will discuss the case when our oracle is noisy, says the oracle $\mathcal{O}_p$. 
%In the original paper \cite{dasarathy2015s2}, they also consider the noisy oracle but they assume that all the queries are not only independent to all the other queries, but also independent to the its own repeated queries. So the technique that they deal with this noisy oracle is repeatedly asking the same query and use majority voting to lower the error probability to desired level. However, as pointed out in \cite{mazumdar2017clustering}, this kind of setting is quite unrealistic. For example, in the crowdsourcing problem, most worker will have a same reference (i.e. the first result from google). Hence the answers from them are not independent and hence the assumption is unrealistic. See more nice discussion in \cite{mazumdar2017clustering}. Instead, when the oracle is able to answer the same cluster queries, \cite{mazumdar2017clustering} proposed a model that the oracle will give the same answer for the repeated query. Hence in this section we will focusing on extending the $S^2$ algorithm under this kind of noisy oracle setting. 

\begin{algorithm2e}
\caption{$S^2$ on hypergraph with noisy pairwise query}\label{alg:S2_noisypair}
\SetAlgoLined
%\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\SetKwRepeat{Do}{do}{while}
\SetKwInOut{Output}{Output}
\SetKwInput{Mainalgo}{Main Algorithm}
\SetKwInput{Phaseone}{Phase 1}
\SetKwInput{Phasetwo}{Phase 2}
  \Input{The graph $G$, query complexity budget $Q(\delta)$, parameter $M$ and the noisy oracle $\mathcal{O}_p$
  }
  \Output{The label function $\widehat{f}$
  }
    \Phaseone{ \\ % Applying algorithm 2 in \cite{mazumdar2017clustering}.\;
        Uniformly at random sample $M$ points from $G$.\;
        Use Algorithm 2 in \cite{mazumdar2017clustering} on these $M$ points to get a partition $\hat{X}_1,...,\hat{X}_k$\;
    }
    \Phasetwo{ \\ % Run $S^2$ algorithm based on the partition $\hat{X}_1,...,\hat{X}_k$\;
        Form a label list $L$ based on $\hat{X}_1,...,\hat{X}_k$\;
        Remove from $G$ all edges whose two ends have different label.\;
        Let $X = \bigcup_{i=1}^{k}\hat{X}_i$, $S = V\setminus X$\;
        \While{1}{
            Uniformly at random sample a point $x$ from $S$\;
            $X\leftarrow S/\{x\}$\;
            \% The above 2 line is not needed if there are $k$ connected components in graph $G' = (V,E\setminus C)$
            \Do{$x\leftarrow MSSP(G,L)$ exist}{
                \If{$x$ is unlabeled}{
                    Query $x$ with all points from $\hat{X}_1,...,\hat{X}_K$, let $A_i$ be the number of "same cluster" queries from $\hat{X}_i$\;
                    Assign $\hat{f}(x) = \arg\max_{i\in [k]}\frac{A_i}{|\hat{X}_i|}$, add this to $L$\;
                }
                Remove from $G$ all edges whose two ends have different label.\;
                \If{$|L|= Q(\delta)$}{
                    Return \emph{LabelComplition}$(G,L)$
                }
            }
        }
    }
\end{algorithm2e}

Now we state our assumption. Basically we assume all the assumption as in section~\ref{sec:scq}. For simplicity we additionally assume that after removing all cut edges, there are exactly $k$ connected components. This assumption can be easily removed and will result a additional term in the bound of query complexity. Basically it will be similar as the first term in theorem \ref{thm:pairwise}.
Moreover, we use the same notation for the noisy oracle as in \cite{mazumdar2017clustering}. Which means the oracle will have probability $p<1/2$ to give the wrong answer. Now we're ready to state the theoretical guarantee for algorithm~\ref{alg:S2_noisypair}.
\begin{theorem}\label{thm:noisycase}
  Suppose the graph $G=(V,E)$ and $f$ are such that the induced cut set $C$ has $m$ cut components that are $\kappa$-clustered. Moreover, there are $k$ underlying cluster in $G$ and there are exactly $k$ connected components in graph $G' = (V,E\setminus C)$. Then for any $\delta>0$ and $p<\frac{1}{2}$, the algorithm~\ref{alg:S2_noisypair} will recover $C$ with probability at least $1-\delta$ if
  \begin{equation*}
    Q(\delta) \geq M^{\dagger}M + \frac{128Mk^2\log M}{(2p-1)^4}
  \end{equation*}
  where
  \begin{align}\label{thm:qcfornoisy}
    M^{\dagger} &= m(\lceil\log_2(n)-\log_2(\kappa)\rceil)\\
    &+ \min(|C|,|\partial C|) (\lceil\log_2(\kappa)\rceil+1)
  \end{align}
  And $M$ is the smallest integer satisfying
  \begin{equation}\label{thm:4req}
    \begin{split}
         & \frac{M}{\log M} \geq \frac{128 k}{\beta (2p-1)^4},\;M \geq \frac{8}{\beta}\log\frac{3k}{\delta},\\
         &\;M \geq \frac{6}{\delta},\;M \geq \frac{2}{\beta D(0.5||p)}\log\frac{6(k-1)M^{\dagger}}{\delta},\;M\leq n/2
    \end{split}
  \end{equation}
  And $D(p||q)$ is the KL-divergence of bernoulli with parameter $p$ and $q$.
\end{theorem}
\begin{remark}
    Note that in the regime the forth requirement of $M$ in \eqref{thm:4req} dominates, we have $M = O(\log(M^{\dagger}))$ where we assume other parameters are constant. Note that this is true when $log(M^{\dagger})$ is large compare to $k$ and $\frac{1}{(2p-1)^4}$, which roughly means the bottleneck of the query complexity is from finding the cut set instead of obtaining the set $X$ in phase 1.
    Then the overall query complexity will be $O(M^\dagger\log(M^{\dagger}))$. Compare to theorem~\ref{thm:pairwise}, we only need additional $O(\log(M^{\dagger}))$ times more queries.
\end{remark}
\begin{remark}\label{rmk:Mleqnhalf}
	Note that the condition $M\leq n/2$ in general will hold when $n$ is sufficiently large. We can still remove this requirement by changing the concentration bound of hypergeometric to the corresponding form (\cite{hoeffding1963probability},\cite{skala2013hypergeometric}). Since in this paper we're interesting in the case that we can efficiently recover the label function with small query complexity, we will only consider the case $M\leq n/2$.
\end{remark}
\begin{remark}
    The assumption "there are exactly $k$ connected components in graph $G' = (V,E\setminus C)$" can be removed. Then we will need more query to make sure that for all connected component in $G' = (V,E\setminus C)$, we at least sample 1 point from each of them. This will cost an additional term $\frac{\log(1/(\beta\delta))}{\log(1/(1-\beta))}$ in $M^{\dagger}$ by the same reason in theorem \ref{thm:pairwise}. Since in the usual application (especially in clustering) the nodes with same label will usually form a connected component, hence for simplicity we only proof the case with assumption "there are exactly $k$ connected components in graph $G' = (V,E\setminus C)$". 
\end{remark}
\begin{remark}
    In fact we can use a slightly looser bound for the forth inequality of \eqref{thm:4req}. It can be replaced by $M \geq \frac{4}{\beta (1-2p)^2}\log(\frac{6(k-1)M^{\dagger}}{\delta})$ because $D(p||q)\geq 2(p-q)^2$ by the convexity of KL divergence. Now we can see that the $\frac{1}{(1-2p)^4}$ term in the first inequality of \eqref{thm:4req} will be larger than $\frac{1}{D(0.5||p)}$ term in the forth inequality of \eqref{thm:4req} more clearly.
\end{remark}
The complete proof of theorem \ref{thm:noisycase} is in the appendix and we only provide the sketch of proof here. Basically the algorithm \ref{alg:S2_noisypair} works as following. The phase 1 of the algorithm \ref{alg:S2_noisypair} recover the labels of $M$ nodes we sampled from $G$ with high probability. This is guarantee by the theorem in \cite{mazumdar2017clustering}. Then in phase 2, we again search for the shortest-shortest path and decide which node to query based on it. We will recover the label of any new node in phase 2 based on the set $X$ we get from phase 1. For a new node need to be query in phase 2, we query it with all the nodes in $X$. We use the "normalized" majority voting to decide the label of that new node. For example when $k=2$, if 10 of 15 queries from $\hat{X}_1$ says the new node $v$ belongs to cluster $\hat{X}_1$ and 15 of 20 queries from $\hat{X}_2$ says the new node $v$ belongs to cluster $\hat{X}_2$, we will assign $v$ with label $2$ since $\frac{15}{20}>\frac{10}{15}$. In the theorem \ref{thm:noisycase} we prove that if $v\in \hat{X}_i$ for some $i\in[k]$, then with high probability the ratio $\frac{A_i}{|\hat{X}_i|}$ will be the largest. Hence our normalized majority voting can recover labels correctly with high probability in phase 2 given the set $X$ are correctly labeled. Also from theorem \ref{thm:pairwise} we know the upper bound of the number of nodes we need to query in order to recover $C$, which is $M^{\dagger}$. Hence the first term in \eqref{thm:qcfornoisy} is correspond to the number of query we need in phase 2, which is $MM^{\dagger}$. The second term in \eqref{thm:qcfornoisy} is correspond to the number of query we need in phase 1, which is by applying the theorem in \cite{mazumdar2017clustering}. Now we explain why we need $M$ to satisfy 5 inequalities in \eqref{thm:4req}. The first inequality is from the requirement of theorem in \cite{mazumdar2017clustering}. The second inequality basically ensures that with high probability we will sample enough points such that $\forall i\in[k],\frac{\hat{X}_i}{|X|}$ is close to $\frac{\sum_{v\in V} \mathbf{1}_{f(v)=i}}{|V|}$, says the true ratio of label $i$. The third inequality is also the result of theorem \cite{mazumdar2017clustering}. The forth inequality is needed because we need to make sure we recover the label of all $M^{\dagger}$ nodes in phase 2. Basically we use union bound among all $M^{\dagger}$ nodes. Finally the fifth inequality is needed because we apply the tail bound for the multivariate hypergeometric distribution. Since we only care about the regime that our algorithm is efficient, the fifth inequality should hold otherwise our algorithm will be mostly running algorithm 2 in \cite{mazumdar2017clustering}. Nevertheless, note that the fifth inequality requirement can be dropped by a more delicate argument, see the discussion in remark \ref{rmk:Mleqnhalf}.

==> simul.tex <==
We performed some preliminary experiments for the $S^2$ algorithm using same-cluster query on some synthetic data, assuming the oracle is noiseless. We used stochastic block model to produce some random graphs containing communities, subsets characterized by being connected with one another with particular edge densities. For simplicity, we set different community to be of equal size and nodes belong to same cluster have the same label. Due to the low probability of nodes being connected from different classes, the clusteredness in terms of cut components($\kappa$-clusterdness) is small. Thus the dominant term in the query complexity(Theorem 4.2) is $k^2\log n$. We ran simulations on stochastic block model with different number of nodes(20 and 40) while keep the rest of parameters to be the same and found out that query complexity grows roughly in the order of $k^2\log n$ which agrees with our theorem. In addition, we also observe that as $n$ increases, the gap between the query complexity in theorem 4.2 and the empirical query complexity tends to vanish. 
\begin{figure}[!htb]
\minipage{0.5\textwidth}
  \includegraphics[width=\linewidth]{new_simul_1.png}
  \caption{Accuracy vs query budget for $n=20$}\label{fig:simul1}
\endminipage\hfill
\minipage{0.5\textwidth}
  \includegraphics[width=\linewidth]{new_simul_2.png}
  \caption{Accuracy vs query budget for $n=40$}\label{fig:simul2}
\endminipage
\end{figure}
For the noisy case and the hypergraph case, the simulations are left for the future work.

==> thmscq1.tex <==
\begin{proof}
The proof for the most parts is exactly the same as the prove given in \cite{dasarathy2015s2}. But for completeness we still include all the proof. The biggest difference compared to the original paper is for same-cluster query you cannot use one simple query to identify the label for one node,  and also the number of runs $R$ can be further tightened according to our argument. The detailed proof is as follows: We  can divide the query complexity in two parts which are associated with the random sampling phase and aggressive search phase. The goal of the random sampling phase is to find a witness to the cut set which implies that we can bound from above the number of random queries needs before can locate a witness set which is done by lemma 4.1. For the aggressive search phase, let $l_{S^2}(G, L, f)$ be the length of the shortest among shortest paths connecting vertices with different labels. After each step of the aggressive search, the $l_{S^2}$ will roughly get halved. Thus it will take no more than $r=\lceil\log_{2}l_{S^2}\rceil +1$ steps to find a cut edge and for each step it will take at most $k$ queries to identify the label of the mid-point. 
In order to bound the required number of active queries, let us split up the aggressive search phase into 'runs', where each run ends when a new boundary vertex has been discovered. Let $R$ be the number of runs, and by definition $R\leq|\partial C|$. For each $i\in R$, let $G_i$ and $L_i$ be the graph and label set up to run $i$. Then the total number of active queries can be upper bounded by $k\sum_{i=1}^{R}(\lceil\log_2(l_{S^2}(G_i, L_i, f))\rceil+1)$.
By observation, in each run it is trivial $l_{S^2}(G_i, L_i, f)\leq n$. In addition, due to the $\kappa$-clusteredness assumption, for arbitrary cut component $C_{rs}$ its undiscovered cut-edge is at most $\kappa$ away from known cut-edge. Thus, for these $|C_{rs}|-1$ runs in $R$, $l_{S^2}\leq\kappa$. And since there are only $m$ cut components, then
\begin{align*}
&k\sum_{i=1}^{R}(\lceil\log_2(l_{S^2}(G_i, L_i, f))\rceil+1)\\
&\leq k(|\partial C|+ m\lceil\log_2 n\rceil +(|\partial C|-m)\lceil\log_2\kappa\rceil)\\
&= km(\lceil\log_2n\rceil-\lceil\log_2\kappa\rceil)+k|\partial C|(\lceil\log_2\kappa\rceil+1)
\end{align*}
On the other hand, the number of runs $R$ can also be upper bounded by $|C|$, since when a new boundary vertex has been discovered if and only if a new cut edge is discovered. Hence we have $R\leq |C|$. Again from the same argument we know that there will be at most $m$ long runs and the rest $R-m$ runs can be bounded according to $\kappa$-clusteredness property. Hence we have
\begin{align*}
&k\sum_{i=1}^{R}(\lceil\log_2(l_{S^2}(G_i, L_i, f))\rceil+1)\\
&\leq k(|C|+ m\lceil\log_2 n\rceil +(|C|-m)\lceil\log_2\kappa\rceil)\\
&= km(\lceil\log_2n\rceil-\lceil\log_2\kappa\rceil)+k|C|(\lceil\log_2\kappa\rceil+1)
\end{align*}
Putting these together we have
\begin{align*}
&k\sum_{i=1}^{R}(\lceil\log_2(l_{S^2}(G_i, L_i, f))\rceil+1)\\
&= km(\lceil\log_2n\rceil-\lceil\log_2\kappa\rceil)+k\min(|C|,|\partial C|)(\lceil\log_2\kappa\rceil+1)
\end{align*}
Hence we complete the proof.
\end{proof}
